Logics with rigidly guarded data tests

The notion of orbit finite data monoid was recently introduced by Bojanczyk as an algebraic object for defining recognizable languages of data words. Following Buchi's approach, we introduce a variant of monadic second-order logic with data equality tests that captures precisely the data languages recognizable by orbit finite data monoids. We also establish, following this time the approach of Schutzenberger, McNaughton and Papert, that the first-order fragment of this logic defines exactly the data languages recognizable by aperiodic orbit finite data monoids. Finally, we consider another variant of the logic that can be interpreted over generic structures with data. The data languages defined in this variant are also recognized by unambiguous finite memory automata.

==> green-theory.tex <==
\subsection{Green's theory and memorable values}\label{app:green-theory}

Here we focus our attention on the memorable values of the elements of orbit finite data monoids.

\begin{definition}\label{def:l-r-values}
Given an element $m$ of an orbit finite data monoid $\cM$, we define by $\memr(s)$
(resp., $\meml(s)$) to be the intersection of $\mem(t)$ for all elements $t$ in the 
$\cR$-class (resp., $\cL$-class) of $s$.
\end{definition}

We call \emph{$\cR$-memorable} (resp., \emph{$\cL$-memorable}) values of $s$ the values 
in $\memr(s)$ (resp., $\meml(s)$).


\medskip
Our final goal is to transform data monoids into rigidly guarded formulas. 
For this, one needs to locate where the memorable data values come from.
An important tool is the following result:

\begin{proposition}\label{prop:memorable-values}
For every element $s$ of an orbit finite data monoid $\cM$, we have
$\mem(s) = \memr(s) \cup \meml(s)$.
\end{proposition}

Before turning to the proof Proposition~\ref{prop:memorable-values}, let us show that 
a similar result fails for data monoids with infinitely many data orbits. Consider the 
data language $L_{\text{even}} \subseteq D^*$ that consists of all words $u\in D^*$ 
where every value $d\in D$ occurs in $u$ an even number of times. The syntactic 
data monoid of the language $L_{\text{even}}$ consists of one element $m_C$ for each
finite subset $C$ of $D$. The product corresponds to the symmetric difference of sets.
It is easy to see that the memorable values  of $m_C$ are exactly the values in $C$,
which are neither $\cL$-memorable nor $\cR$-memorable (the data monoid is a group).

In order to prove Proposition \ref{prop:memorable-values}, we need to introduce a couple of 
other concepts. An \emph{inverse} of an element $s$ of a monoid, is an element $t$ such 
that $s\cdot t=t\cdot s=1_\cM$. If the inverse of $s$ exists, then it can be easily 
proven to be unique and hence it can be denoted by $s^{-1}$. A \emph{data group} is 
simply a \emph{data monoid} where all elements have an inverse. The next lemma shows 
that orbit finiteness is, quite surprisingly, a severe restriction for data groups.

\begin{lemma}\label{lemma:data-groups}
Every orbit finite data group is finite.
\end{lemma}     

\begin{proof}
We first observe that:

\begin{claim}
{\bf Claim 1.} 
In an orbit finite data group, $\mem(s)=\mem(s^{-1})$.
\end{claim}

\begin{proof}[Proof of Claim 1.]
Since orbit finite data groups are locally finite, there is $n>0$ such that $s^n=1$ 
and hence $s^{-1}=s^{n-1}$. This implies $\mem(s^{-1})=\mem(s^{n-1})\subseteq\mem(s)$.
By symmetry, we get $\mem(s)=\mem(s^{-1})$.
\end{proof}

\begin{claim}
{\bf Claim 2.}
$\mem s\setminus\mem t\subseteq \mem(s\cdot t)$.
\end{claim}

\begin{proof}[Proof of Claim 2.]
Indeed, $\mem(s)=\mem(s\cdot t\cdot t^{-1})\subseteq\mem(s\cdot t)\cup\mem(t^{-1})=\mem(s\cdot t)\cup\mem(t)$.
Hence, $\mem(s)\setminus\mem(t)\subseteq\mem(s\cdot t)$.
\end{proof}

Now, assume, towards a contradiction, that $\cG$ is an infinite data group 
with finitely many orbits. $\cG$ must contain an infinite orbit $o$. Let
$H=\{h_1, h_2, \ldots\}$ be some infinite subset of $o$ such that each element $h_i$ has a 
distinguished memorable value $d_i$ that is not memorable in any other element of $H$.
Then, from the above claim, for all $k$, $\{d_1,\dots,d_k\}\subseteq\mem(s_1\cdots s_k)$.
This contradicts the finite memory property.
\end{proof}

It is know that every $\cH$-class $H$ of a monoid is associated with a group $\Gamma(H)$ called the 
Sch\"utzenberger group \cite{mathematical_foundations_of_automata} (in fact there exist two such 
groups, but we will only consider one of them here). We define $T(H)$ to be the set of all elements 
$t \in H$ such that $t\cdot H$ is a subset of $H$. For each $t\in T(H)$ we let $\gamma_t$ be the 
transformation on $H$ that maps $h\in H$ to $t\cdot h$. Formally the Sch\"utzenberger group $\Gamma(H)$ 
consists of the set of all transformations $\gamma_t$ with $t\in T(H)$. The multiplication operation 
of the group is the functional composition $\circ$. Moreover, there is a natural way to extend the 
action $\hat\blank$ of the data monoid $\cM$ to an action $\tilde\blank$ on $\Gamma(H)$ by simply 
letting $\tilde\tau(\gamma_s) = \gamma_{\hat{\tau}(s)}$ for all renamings 
$\tau\in\Gamma_{D \setminus (\memr(H)\cup\meml(H))}$, where $\memr(H)=\memr(h)$ 
and $\meml(H)=\meml(h)$ for some arbitrary element $h\in H$ (note that all elements 
of $H$ have the same set of $\cR$-memorable values and the same set of $\cL$-memorable 
values). The following lemma shows that $\tilde\blank$ is indeed a group action on 
the Sch\"utzenberger group $\Gamma(H)$.

\begin{lemma}\label{lemma:schutzenberger-data-group}
If $\cM=(M,\cdot,\hat\blank)$ is a data monoid over the set $D$ of data values and $H$ is an $\cH$-class of $\cM$, 
then $(\Gamma(H),\circ,\tilde\blank)$ is a data group over the set $D\setminus (\memr(H)\cup\meml(H))$.
Moreover, if $\cM$ is orbit finite, then $(\Gamma(H),\circ,\tilde\blank)$ is orbit finite as well.
\end{lemma}

\begin{proof}
It is known that $(\Gamma(H),\circ)$ is a group. We only need to verify that $\tilde\blank$ is an action on $\Gamma(H)$. We first show that $\Gamma(H)$ is closed
under the action $\tilde\blank$ of the renamings over $D\setminus (\memr(H)\cup\meml(H))$. By 
definition of $\tilde\blank$, this is equivalent to verifying that $H$ is closed under the action 
$\hat\blank$ of renamings over $D\setminus (\memr(H)\cup\meml(H))$. The following proof is similar 
to proof of the Memory Theorem for $\cJ$-classes in \cite{data_monoids}; however, we give a complete
proof here for the sake of self-containment. 

Suppose that $H$ is the intersection of an $\cR$-class $R$ and an $\cL$-class $L$. As a renaming is a permutation that is the identity on all but finite many values, any renaming over $D\setminus (\memr(H)\cup\meml(H))$ can be decomposed into 
a sequence of transpositions of pairs of values from $D\setminus (\memr(H)\cup\meml(H))$. 
Therefore, in order to prove the closure of $H=R\cap L$ under the action of the renamings over 
$D\setminus (\memr(H)\cup\meml(H))$, it is sufficient to prove a similar closure property for
the transpositions $\pi_{de}$ of pair of elements $d,e\nin\memr(H)\cup\meml(H)$. We first show 
that $R$ is closed under such transpositions. Let $d$ and $e$ be two values outside $\memr(H)$ 
and let $\pi_{de}$ be their transposition. Since $d,e\nin\memr(H)$, we know that there exist 
two elements $s,t\in R$ such that $d$ is not memorable in $s$ and $b$ is not memorable in $t$. 
Let $f$ be a value outside $\mem(s) \cup \mem(t)$. By definition of memory, we know that $\hat\pi_{df}$, 
where $\pi_{df}$ is the transposition of $d$ and $f$, is a stabilizer of $s$ and, similarly, $\hat\pi_{ef}$ 
is a stabilizer of $t$. Now, consider an element $s'$ that is $\cR$-equivalent to $s$. There must 
exist $u$ and $u'$ in $\cM$ such that $s\cdot u=s'$ and $s'\cdot u'=s$. Since $\hat\blank$ commutes 
with the product of $\cM$, we obtain $\hat\pi_{df}(s')=\hat\pi_{df}(s\cdot u)$ and hence 
$\hat\pi_{df}(s') \le_{\cR} \hat\pi_{df}(s)$. By similar arguments, we obtain 
$\hat\pi_{df}(s') \ge_{\cR} \hat\pi_{df}(s)$. We thus have $\hat\pi_{df}(s') \gR \hat\pi_{df}(s) = s \in R$. 
A symmetric argument shows that $\hat\pi_{ef}(s') \gR \hat\pi_{ef}(s) = s \in R$. Since 
$\pi_{de}=\pi_{df}\circ\pi_{ef}\circ\pi_{df}$, we conclude that $\hat\pi_{de}(s) \in R$.
Finally, a similar proof shows that $\hat\pi_{de}(s) \in L$. Putting all together, we have 
that for every $s\in H=R\cap L$ and every renaming $\tau$ over $D\setminus (\memr(H)\cup\meml(H))$,
$\hat\tau(s)\in R\cap L=H$. This shows that $H$ is closed under the action $\hat\blank$ of renamings
over $D\setminus (\memr(H)\cup\meml(H))$.

Below, we verify that $\tilde\blank$ is a group morphism from the group of renamings $G_{D\setminus (\memr(H)\cup\meml(H))}$
to the group of automorphisms on $\Gamma(H)$. Clearly, the function $\tilde\blank$ maps the identity 
$\iota$ on $G_{D\setminus (\memr(H)\cup\meml(H))}$ to the trivial automorphism $\tilde\iota$ on $\Gamma(H)$ 
(i.e., $\tilde\iota(\gamma_s)=\gamma_{\hat\iota(s)}=\gamma_s$). Moreover, $\tilde\blank$ is a morphism 
because
$$
  \widetilde{\tau \circ \pi}(\gamma_s) \;=\;
  \gamma_{\widehat{\tau \circ \pi}(s)} \;=\;
  \gamma_{\hat\tau \circ \hat\pi(s)} \;=\;
  (\tilde\tau \circ \tilde\pi)(\gamma_s).
$$
Finally, we observe that $\gamma_{s \cdot t} = \gamma_s \circ \gamma_t$ (indeed, for every $h\in H$, we have
$\gamma_{s \cdot t}(h) = (s \cdot t) \cdot h = s \cdot (t \cdot h) = \gamma_s(t \cdot h) = \gamma_s \circ \gamma_t(h)$)
and hence
$$
  \hat{\tau}(\gamma_s) \circ \hat{\tau}(\gamma_t) \;=\; 
  \gamma_{\hat{\tau}(s)} \circ \gamma_{\hat{\tau}(t)} \;=\; 
  \gamma_{\hat{\tau}(s) \cdot \hat{\tau}(t)} \;=\; 
  \gamma_{\hat{\tau}(s \cdot t)} \;=\; \hat{\tau}(\gamma_{s \cdot t}) \;=\;
  \hat{\tau}(\gamma_s \circ \gamma_t).
$$

\noindent
To complete the proof of the lemma, we need to prove that $(\Gamma(H),\circ,\tilde\blank)$ is orbit finite
when $\cM$ is orbit finite. Let us consider two elements $s,t \in H$ and suppose that $s$ and $t$ are in the 
same orbit, namely, that there is $\tau\in G_{D\setminus (\memr(H)\cup\meml(H))}$ such that $t=\hat\tau(s)$. 
Since $\tilde\blank$ is a group action, we know that $\gamma_t=\gamma_{\hat\tau(s)}=\tilde\tau(\gamma_s)$. 
This shows that the two elements $\gamma_s$ and $\gamma_t$ of $\Gamma(H)$ are on the same orbit.
\end{proof}     

It is known that any $\cH$-class $H$ of a 
monoid has the same cardinality of the associated Sch\"utzenberger group $\Gamma(H)$.
Hence, we obtain the following interesting property:

\begin{corollary}\label{cor:finite-H-classes}
All $\cH$-classes of an orbit finite data monoid are finite.
\end{corollary}

\begin{proof}
Let $H$ be an $\cH$-class of an orbit finite data monoid $\cM$. By Lemma \ref{lemma:schutzenberger-data-group}, 
we can associate with $H$ an orbit finite data group $(\Gamma(H),\circ,\tilde\blank)$, where $\Gamma(H)$ is 
the Sch\"utzenberger group of $H$. By Lemma \ref{lemma:data-groups}, it follows that $\Gamma(H)$ is finite.
Moreover, it is known from classical results in algebra (see, for instance, \cite{mathematical_foundations_of_automata}),
that the Sch\"utzenberger group $\Gamma(H)$ has the same cardinality as the $\cH$-class $H$. We thus conclude that
$H$ is finite.
\end{proof}

We are now ready to prove Proposition~\ref{prop:memorable-values}.

\begin{proof}[Proof of Proposition \ref{prop:memorable-values}]
We aim at $\mem(s)\subseteq\memr(s) \cup \meml(s)$. Assume towards 
a contradiction that there is a value $d \in \mem(s)\setminus( \memr(s) \cup \meml(s))$. As $d\nin\memr(s)$, 
there is an $s'$ in the $\cR$-class of $s$ such that $d\nin\mem(s')$. Then 
there are $u,u' \in     \cM$ such that $s\cdot u=s'$ and $s'\cdot u'=s$. 
Symmetrically, as $d\nin\meml(s)$, $s$ has an $\cL$-equivalent element $s''$ 
such that $d\nin\mem(s'')$, and there are  $v,v'' \in \cM$ such that $v\cdot s=s''$ and $v''\cdot s''=s$. 

Let $d_1,d_2,\ldots$ be an infinite sequence of pairwise distinct values that are not in the memory of either 
$s$, $s'$, or $s''$. We denote by $\pi_i$ the transposition of $d$ with $d_i$. As neither $d$ nor $d_1,d_2,\ldots$ are in the 
memory of $s'$, $\hat\tau_i(s')=s'$ and hence $\hat\tau_i(s\cdot u)=\hat\tau_i(s')=s'$. 
Combining this with $s'\cdot u'=s$ we obtain $\hat\tau_i(s)\cdot\hat\tau_i(u)\cdot u' = s'\cdot u' = s$ and hence $\hat\tau_i(s) \ge_{\cR} s$. Similarly, one proves that $\hat\tau_i(s) \le_{\cR} s$ and 
hence $\hat\tau_i(s) \gR s$. By symmetry 
$\hat\tau_i(s) \gL s$. Hence $\hat\tau_i(s)$ belongs to the 
$\cH$-class of $s$. As $d$ is memorable in $s$, $\hat\tau_i(s)$ is different from $s$. Thus the $\cH$-class of $s$
is infinite, contradicting Corollary \ref{cor:finite-H-classes}.
\end{proof}



==> logics-for-automata__backup_for_trees_.tex <==
\section{Logics for finite memory automata on data trees}\label{sec:logics-for-automata}

In this section, we consider again variants of \MSO with guards on data tests.
More precisely, we consider the logic \emph{semi-rigidly guarded \MSO}, as it 
was introduced in Section \ref{sec:logics}, but now we interpret it over the 
class of (finite ranked) data trees. The goal is to relate definability in 
semi-rigidly guarded \MSO to recognizability of languages of data trees by 
means of finite memory automata 
\cite{finite_memory_automata,nondeterministic_reassignment,finite_memory_automata_on_trees}. 

We recall that, in semi-rigidly guarded \MSO, every data test $y\sim z$ 
is put in conjunction with a formula $\alpha(x,y) ~\et~ \beta(x,z)$, where 
$\alpha(x,y)$ (resp., $\beta(x,z)$) is a formula of semi-ridigly guarded \MSO
that defines at most one position $y$ (resp., $z$) from each position $x$.
We also recall below one of the possible alternative definitions for finite memory 
automata on data trees, precisely the one from \cite{automata_with_group_actions}, 
which is the closest one in spirit to orbit-finite data monoids. For this we will
reuse some notions from Section \ref{sec:background}, in particular, that of 
$\cG_D$-set and that of equivariant subset. 
Hereafter, all elements in a $\cG_D$-set are tacitly assumed to have finite memory. 
For simplicity, we will also avoid denoting explicitly the group actions underlying
$\cG_D$-sets.

\begin{definition}\label{def:finite-memory-automaton}
A \emph{finite memory automaton} (\emph{FMA} for short) is a tuple $\cA=(\Sigma,Q,F,T)$, 
where:
\begin{itemize}
  \item $\Sigma$ is an orbit-finite $\cG_D$-set that plays the role of the input alphabet 
        (e.g. $D\times A$); every element $c\in\Sigma$ has an associated \emph{arity},
        denoted $\arity(c)$, that is invariant under the action of renamings, namely,
        $\arity(\tau(c)) = \arity(c)$, and that determines the number of children under
        any $c$-labelled node;
  \item $Q$ is an orbit-finite $\cG_D$-set that plays the role of the configuration space;
  \item $F$ is an equivariant subset of $Q$, i.e.~a union of orbits of $Q$, that 
        contains the configurations that can be associated with the root of a tree
        in a successful run;
  \item $T$ is an equivariant subset of $\bigcup_{c\,\in\Sigma} Q\times\{c\}\times Q^{\arity(c)}$
        that describes the possible configurations that can be associated with 
        a $c$-labelled node and its children.
\end{itemize}
The notion of \emph{successful run} of $\cA$ and that of \emph{recognized language} 
are the usual ones for automata running on finite ranked trees (they are just 
generalized to possibly infinite alphabets and configuration spaces).
The FMA $\cA=(\Sigma,Q,F,T)$ is said to be
\begin{enumerate}
  \item \emph{unambiguous}, 
        if it admits at most one successful run on each input data tree;
  \item \emph{bottom-up deterministic}, 
        if $(q,c,q_1,\ldots,q_h),(q',c,q_1,\ldots,q_h) \in T_a$ implies $q=q'$;
  \item \emph{top-down deterministic}, 
        if $F$ contains a single configuration with empty memory and 
        $(q,c,q_1,\ldots,q_h),(q,c,q'_1,\ldots,q'_h) \in T_a$ implies $q_j=q'_j$ 
        for all $j=1,\ldots,h$.
\end{enumerate}
\end{definition}

FMA can be easily shown to be closed under union and intersection (the classical 
constructions for finite state automata can be used). In addition, bottom-up deterministic
FMA and top-down deterministic FMA are closed under complementation. However, FMA
are not closed under projections and cannot be determinized in general.
We can also think of a data word as a unary tree where the first position corresponds 
to the unique leaf (for this, we assume, without loss of generality, that there is a 
special symbol of arity $0$ that marks the beginning of a data word). Accordingly,
we have that FMA are at least as expressive as orbit-finite data monoids. In fact, 
FMA (even bottom-up or top-down deterministic ones) are strictly more expressive 
than orbit-finite data monoids, even when operating on data words. For example, 
a separating language is
$$
  L_\curvearrowright ~~\eqdef~ \{d_1\ldots d_n ~:~ n\in\bbN,~d_1=d_i \text{ for some $1<i\le n$}\}
$$
which is recognized by a bottom-up deterministic FMA, but is not recognizable by an 
orbit-finite data monoid. Moreover, unlike classical finite automata, bottom-up
deterministic FMA are incomparable with top-down deterministic FMA, and both are
strictly less expressive than unambiguous FMA, as easily witnessed by the
language $L_\curvearrowright$ and its reverse.

With the lack of classical tools like the subset construction, the problem of finding 
logical characterizations of classes of data languages recognized by FMA becomes challenging. 
In the following, we give partial results towards this goal.


\medskip
The first result shows that FMA, even unambiguous ones, are at least as expressive
as semi-rigidly guarded \MSO interpreted on data trees.

\begin{theorem}\label{th:semi-rigid-inside-fma}
Every language of data trees defined by a semi-rigidly guarded \MSO sentence 
is effectively recognized by an unambiguous FMA.
\end{theorem}

\begin{proof}
To translate a sentence $\psi$ of semi-rigidly guarded \MSO into an equivalent
unambiguous FMA $\cA_\psi$, it is convenient to first normalise $\psi$ into a 
sentence $\psi'$ that contains no nested data tests. We do so by using an approach 
similar to the proof of Theorem \ref{thm:decidability}, namely, we substitute in 
$\psi$, starting from the innermost subformulas, every occurrence of a semi-rigidly 
guarded data test 
$\varphi(x,y,z) \:=\: \alpha(x,y) \:\et\: \beta(x,z) \:\et\: y\sim z$, 
with the formula 
$\varphi^*(x,y,z) \:=\: \alpha^*(x,y) \:\et\: \beta^*(x,z) \:\et\: x\in c_{\alpha,\beta}^\sim$,
where $c_{\alpha,\beta}^\sim$ is a fresh unary predicate associated with that occurrence.
Note that, by the inductively defined transformation, none of the guards $\alpha^*,\beta^*$ 
contain data tests, and hence $\varphi^*(x,y,z)$ can be seen as a sentence of classical MSO 
over a signature extended with monadic predicates $c^\sim_{\alpha,\beta}$.
We let $C$ be the set of all predicates $c^\sim_{\alpha,\beta}$ and we conjoin 
the MSO sentence $\psi^*$ with sentences of the form
$$
  \phi_{c_{\alpha,\beta}^\sim} ~\eqdef~
  \exists c_{\alpha,\beta}^\sim ~ \forall x ~ 
  \big(\, x\in c_{\alpha,\beta}^\sim ~\leftrightarrow~ 
                  \exists y,z ~ 
                  \alpha^*(x,y) \:\et\: \beta^*(x,z) \:\et\: y\sim z \,\big)
$$
for each $c_{\alpha,\beta}^\sim\in C$.
It is immediate to see that the sentence 
$\psi' \:\eqdef\: \psi^* \,\et~ \bigwedge_{c_{\alpha,\beta}^\sim} \phi_{c_{\alpha_\beta}^\sim}$
is equivalent to the original sentence $\psi$. Moreover, $\psi'$ has a simple form 
with no nested data tests, which eases the translation towards unambiguous FMA. 
In particular, the first subformula $\psi^*$ can be easily translated into a 
finite state automaton $\cA_{\psi^*}$. Below, we describe in detail how to translate
the remaining sentences $\phi_{c_{\alpha_\beta}^\sim}$ into unambiguous FMA.
After this, one can simply exploit closure under intersection to obtain an 
unambiguous FMA $\cA_{\psi'}$ equivalent to $\psi'$, and hence to $\psi$. 

Let us consider a sentence $\phi_{c_{\alpha,\beta}^\sim}$. 
We start by translating the semi-rigid MSO guard $\alpha^*(x,y)$.
\gabriele{Could be a sibling!}
Without loss of generality we can assume that $\alpha^*(x,y)$ either 
always entails that $x$ is an ancestor of $y$, or entails that $x$ is 
a descendant of $y$ -- if this were not the case, we could simply write 
$\alpha^*(x,y)$ as a disjunction $\alpha_1^*(x,y) \vel \alpha_2^*(x,y)$
of two semi-rigid formulas satisfying the assumption, and then distinguish 
the positions $x\in c^\sim_{\alpha,\beta}$ depending on whether 
$\alpha_1^*(x,y)$ or $\alpha_2^*(x,y)$ holds, where $y$ is uniquely
determined from $x$.
Since $\alpha^*(x,y)$ is an MSO formula, we can
easily translate it to a bottom-up deterministic finite tree automaton 
$\cB_\alpha$ over the alphabet $A\times C\times B^3$, where the three
copies of the binary alphabet $B$ are used to encode the variables $x$, $y$,
and $z$. Let $Q_\alpha$
\gabriele{Change everything from here!}

%
%Moreover, depending on whether $\alpha^*(x,y)$ entails that $x$ is an 
%ancestor of $y$, or conversely, we assume that $\cB_\alpha$ is bottom-up
%deterministic, or top-down deterministic.

Similarly, we construct a bottom-up deterministic finite tree 
automaton $\cB_\beta$
\end{proof}

\noindent\hrulefill

The proof uses techniques similar to those of Theorem \ref{thm:formula-to-monoid}. 
Specifically, it exploits closure properties of suitable forms of FMA under 
complementation (corresponding to the negation of a formula), intersection 
(corresponding to conjunction of formulas), and projection (corresponding to 
existential quantification). To be able to prove these closure properties,
however, we need to be precise about the class of automata that we manipulate.
Intuitively, these automata are unambiguous FMA obtained from cascade products 
of bottom-up deterministic and top-down deterministic FMA. Below, we give the 
definition of a form of cascade product and state some of its basic properties; 
for further details, we refer the reader to 
\cite{algebraic-theory-of-machines,theory-of-automata-networks}.

\begin{definition}\label{def:cascade-product}
Let $\cA_1=(\Sigma_1,Q_1,F_1,T_1)$ and $\cA_2=(\Sigma_2,Q_2,F_2,T_2)$ be two FMA, 
where $\Sigma_2=\Sigma_1\times Q_1$ and $\arity(c,q)=\arity(c)$ for all $(c,q)\in\Sigma_2$. 
The \emph{cascade product} of $\cA_1$ and $\cA_2$ is defined as the FMA 
$\cA_1 * \cA_2 = (\Sigma_1,Q,F,T)$, where $Q=Q_1\times Q_2$, $F=F_1\times F_2$, 
and $T$ consists of all and only the tuples of the form $((q,q'),c,(q_1,q'_1),\ldots,(q_h,q'_h))$, 
with $h=\arity(c)$, $(q,c,q_1,\ldots,q_h)\in T_1$, and $(q',(c,q),q'_1,\ldots,q'_h)\in T_2$.
\end{definition}

The operation of cascade product is associative and preserves unambiguity, bottom-up 
determinism, and top-down determinism. Hereafter, we tacitly assume that all cascade 
products are of the form $\cA_1*\ldots*\cA_\ell$, with each FMA $\cA_i$ being either
bottom-up deterministic or top-down deterministic. Note that the FMA that result
from these cascade products are unambiguous. 

When implementing the operations of complementation, intersection, and projection on the 
recognized data languages, we will manipulate directly the automata that form our cascade 
products. For example, it is easy to implement the operation of complementation of a data 
language recognized by $\cA_1*\ldots*\cA_\ell$, as it suffices to complement each deterministic
FMA $\cA_i$. Similarly, the operation of intersection of two data languages recognized 
by $\cA_1*\ldots*\cA_\ell$ and $\cA'_1*\ldots*\cA'_{\ell'}$ is performed as follows. 
Without loss of generality, namely, by inserting dummy automata, we can assume that 
the two cascade products have the same length and have automata of the same kind at 
each level, namely, for every $1\le i\le \ell=\ell'$, either $\cA_i$ and $\cA'_i$ 
are bottom-up deterministic, or they are top-down deterministic. 
Under this assumption, the intersection operation is implemented component-wise
by computing products of each pair of automata $\cA_i$ and $\cA'_i$.

Let us now consider the operation of projection. In general, this operation introduces 
some ambiguity, even at the level of the single deterministic automata (recall that a 
similar issue occurred when considering projections of languages recognized by orbit-finite 
data monoids). We solve this problem by further restricting the types of cascade products,
in a way that is similar to the notion of projectability for data monoid morphisms 
(see Section \ref{sec:logic2monoids}). 
As usual, $B$ denotes the binary alphabet $\{0,1\}$ and the symbols in the expanded
alphabet $A\times B^m$ inherit their arities from the symbols of $A$. We use $\bar{U}$
as a shorthand for a tuple of unary predicates $U_1,\ldots,U_m$.

\begin{definition}\label{def:projectable-fma}
A cascade product $\bar{\cA}=\cA_1*\ldots*\cA_\ell$ recognizing a data language over 
the alphabet $D\times A\times B^m$ is said be \emph{projectable} (\emph{over $B^m$}) if
\begin{itemize}
  \item every automaton $\cA_i$ is bottom-up deterministic or top-down deterministic;
  \item for every data tree $\ang{t,\bar{U}}$, 
        the FMA resulting from $\bar{\cA}$ admits a (necessarily unique, possibly not 
        successful) run on $\ang{t,\bar{U}}$, which is hereafter denoted 
        by $\bar{\cA}\ang{t,\bar{U}}$ and is seen as a function mapping 
        nodes $x$ to configurations $\bar{\cA}\ang{t,\bar{U}}(x)$;
  \item for any two expansions $\ang{t,\bar{U}}$ and $\ang{t,\bar{V}}$ 
        of the same data tree $t$ over $D\times A$, we have
        $$
          \qquad
          \bar{\cA}\ang{t,\bar{U}}(x) ~\orbiteq~ \bar{\cA}\ang{t,\bar{V}}(x)
          \quad\text{implies}\quad
          \bar{\cA}\ang{t,\bar{U}}(x) ~=~ \bar{\cA}\ang{t,\bar{V}}(x)
        $$
        (recall that $q \orbiteq q'$ means that the two configurations $q$ and $q'$ 
         are in the same orbit).
\end{itemize}
%
%An FMA $\cA$ over the alphabet $D\times A\times B^m$ is \emph{bottom-up projectable} 
%(resp., \emph{top-down projectable}) if it is bottom-up deterministic (resp., top-down 
%deterministic), it admits a necessarily unique (possibly not successful) run 
%$\cA(\ang{t,\bar{U}})$ on every input data tree $\ang{t,\bar{U}}$, and, for all 
%data trees $\ang{t,\bar{U}}$ and $\ang{t,\bar{V}}$ and all nodes $x$, we have
%$$
%  \cA(t,\bar{U})(x) ~\orbiteq~ \cA(t,\bar{V})(x)
%  \qquad\text{implies}\qquad
%  \cA(t,\bar{U})(x) ~=~ \cA(t,\bar{V})(x) \ .
%$$
\end{definition}

\noindent
We remark that, given a projectable cascade product $\bar{\cA}=\cA_1*\ldots*\cA_\ell$, 
every prefix $\cA_1*\ldots*\cA_i$ of it is also projectable. Moreover, note that the 
closure properties under complementation and intersection can be immediately transferred 
to projectable cascade products. Below, we prove that the latter are also closed under 
projections.

\begin{lemma}\label{lemma:projectable-fma}
Projectable cascade products of FMA are effectively closed under projections.
\end{lemma}

\begin{proof}
For the sake of simplicity, we consider only projections from the alphabet $D\times A\times B$
to the alphabet $D\times A$. Let $L\subseteq (D\times A\times B)^*$ be a data language recognized 
by a projectable cascade product $\bar{\cA} = \cA_1*\ldots*\cA_\ell$. We aim at constructing 
a new projectable cascade product $\bar{\cA}' = \cA'_1*\ldots*\cA'_\ell$ that recognizes the 
language
$$
  L' ~~\eqdef~~ \big\{\, t ~:~ \exists\, U\subseteq\dom(t).~ \ang{t,U}\in L \,\big\} \ .
$$
To construct the automata $\cA'_i$ that form the desired cascade product, we will exploit 
variants of the subset construction that simulate several transitions of the automata $\cA_i$
from the original cascade product. As usual, we need to avoid storing too many configurations 
inside a macro-state of the subset construction, as this may result in a configuration space 
with an infinite number of orbits. Such a construction will turn out to be feasible thanks 
to the projectability assumption. Formally, we assume that the $i$-th component of the 
cascade product recognizing $L$ is an FMA of the form $\cA_i=(\Sigma_i,Q_i,F_i,T_i)$, 
where $\Sigma_i \:=\: D\times A\times B\times Q_{i-1}$, and we define 
$\cA'_i=(\Sigma'_i,Q'_i,F'_i,T'_i)$ by induction on $i$, as follows:
\begin{itemize}
  \item $\Sigma'_i \:=\: D\times A\times Q'_{i-1}$, under the convention
        that $Q'_0$ is the set containing a single dummy configuration;
  \item the configurations in $Q'_i$ are the subsets of $B\times Q_i$ 
        that contain only pairwise orbit-distinct elements, namely, 
        the sets $S\subseteq B\times Q_i$ such that $(b,q),(b,q')\in S$ 
        and $q=\tau(q')$ imply $q=q'$; 
        we lift in the natural way the group action on $Q_i$ 
        to a group action on $Q'_i$ and we think of $Q'_i$ as a $\cG_D$-set;
        we also observe that the configurations in $Q'_i$ have memories of 
        size uniformly bounded by the numbers of orbits of $Q_i$ 
        and hence $Q'_i$ has only finitely many orbits;
  \item $F'_i$ contains those sets $S\in Q'_i$ such that $S \cap (B\times F_i) \neq \emptyset$;
        it is easy to see that $F'_i$ is an equivariant subset of $Q'_i$;
  \item to define the transitions in $T'_i$ we need to distinguish two cases
        depending on whether $\cA_i$ is bottom-up deterministic or top-down deterministic:
        \begin{enumerate}
          \item if $\cA_i$ is bottom-up deterministic, then $T'_i$ contains 
                all and only the tuples $(S,C,S_1,\ldots,S_h)$ such that 
                $S,S_1,\ldots,S_h\in Q'_i$, $C=(d,a,S')\in\Sigma'_i$ 
                ($=D\times A\times Q'_{i-1}$), $h=\arity(a)$, and
                $$
                  \qquad
                  S ~=~ \left\{\, (b,q) ~: \begin{array}{l}
                                             (q,c,q_1,\ldots,q_h)\in T_i,~
                                             c = (d,a,b,q') \in \Sigma_i,~ \\
                                             (b,q')\in S',~
                                             (b_1,q_1)\in S_1, \ldots, (b_h,q_h)\in S_h
                                           \end{array} 
                        \,\right\}
                $$
          \item if $\cA_i$ is top-down deterministic, then $T'_i$ contains 
                the tuples $(S,C,S_1,\ldots,S_h)$ such that 
                $S,S_1,\ldots,S_h\in Q'_i$, $C=(d,a,S')\in\Sigma'_i$ 
                ($=D\times A\times Q'_{i-1}$), $h=\arity(a)$, and, 
                finally, for every $j=1,\ldots,h$,
                $$
                  \qquad\quad
                  S_j ~=~ \left\{\, (b_j,q_j) ~: \begin{array}{l}
                                                   (q,c,q_1,\ldots,q_h)\in T_i,~
                                                   c = (d,a,b,q') \in \Sigma_i,~ \\
                                                   (b,q')\in S',~
                                                   (b,q)\in S
                                                 \end{array} 
                          \,\right\} \ .
                $$
        \end{enumerate}
\end{itemize}
It is easy to see from the above definitions that if $\cA_i$ is bottom-up deterministic
(resp., top-down deterministic), then so is $\cA'_i$.
To prove that the cascade product $\bar{\cA}' = \cA'_1*\ldots*\cA'_\ell$ is projectable 
and recognizes the projection of the language recognized by $\bar{\cA}$, we need to 
analyse in detail the runs of each automaton $\cA_i$ that can be induced by some 
computations of the cascade product $\bar{\cA}$ on the input data trees of the form 
$\ang{t,U}$, with $U\subseteq\dom(t)$, and do similarly for the cascade product 
$\bar{\cA}'$. For this we need to introduce some notation. 

We recall that $\bar{\cA}$ is projectable and hence it admits a unique run 
$\bar{\cA}\ang{t,U}$ on each input data tree $\ang{t,U}$. Given $1\le i\le\ell$, 
we denote by $\bar{\cA}\ang{t,U}[i]$ the projection of this run onto the configurations 
of $\cA_i$, and we think of it as the run of $\cA_i$ induced by the data tree $\ang{t,U}$ 
and by the corresponding runs of $\bar{\cA}\ang{t,U}[1]$, $\ldots$, $\bar{\cA}\ang{t,U}[i-1]$ 
for the automata in the lower levels of the cascade product. 
Analogous observations hold for the runs of the automata $\cA'_1,\ldots,\cA'_\ell$, 
with the only exception that we need to preliminarily verify the existence of these runs. 
By a slight abuse of notation, we denote by $\ang{t,\rho}$ the data tree obtained by annotating
$t$ with some run $\rho$, provided that $\dom(t)=\dom(\rho)$ (note that $\rho$ is not, strictly 
speaking, a unary predicate). 
In the following claim, we formalise a invariant for the computations of the automata 
in a partial cascade product of the form $\cA'_1*\ldots*\cA'_i$. We will see later how 
such an invariant can be used to prove that the cascade product 
$\bar{\cA}' = \cA'_1,\ldots,\cA'_\ell$ is projectable and recognizes 
the desired language.

\begin{claim}\label{claim:fma-subset-construction}
For every $0\le i\le\ell$ and every data tree $t$, the FMA $\cA'_1,\cA'_2,\ldots,\cA'_i$ 
admit (necessarily unique) runs $\rho_1,\rho_2,\ldots,\rho_i$ on the data trees $t$, 
$\ang{t,\rho_1}$, $\ldots$, $\ang{t,\rho_{i-1}}$ such that, for all indices $1\le j\le i$ 
and all nodes $x$,
\begin{align*}
  \rho_j(x) ~=~ \big\{\, \bar{\cA}\ang{t,U}[j](x) ~:~ U\subseteq\dom(t) \,\big\} \ .
  \tag{$\star$}
\end{align*} 
\end{claim}

\begin{proof}[Proof of claim]
The proof is by induction on $i$, where the base case $i=0$ holds trivially. 
To prove the inductive step, we assume that the claim holds for $i-1$ and we 
prove it for $i$. In the following, we often refer to a tree of the form
$\ang{t,\rho_{i-1}}$, where $\rho_{i-1}$ is a run of $\cA_{i-1}$: this makes
sense only if $i>1$; in the specific case where $i=1$, we simply think of 
$\ang{t,\rho_{i-1}}$ as the tree $t$ itself.

We begin by considering the case where $\cA_i$ is bottom-up deterministic. 
Let $\rho_1,\ldots,\rho_{i-1}$ be the runs of $\cA'_1,\cA'_2,\ldots,\cA'_{i-1}$
on the trees $t$, $\ang{t,\rho_1}$, $\ldots$, $\ang{t,\rho_{i-2}}$, respectively, 
that satisfy equation ($\star$) for all $1\le j\le i-1$. We can construct the
desired run $\rho_i$ of $\cA'_i$ on the tree $\ang{t,\rho_{i-1}}$ that will
prove the inductive step by exploiting a simple structural induction, namely, 
by defining the configurations $\rho_i(x)$ on all nodes $x$, starting from the 
leaves and going upward. More precisely, consider a node $x$ in the data tree 
$\ang{t,\rho_{i-1}}$ and let $x_1,\ldots,x_h$ be its children (possibly $h=0$). 
Suppose that some partial runs of $\cA'_i$ on the subtrees rooted at $x_1,\ldots,x_h$ 
have been defined, and let $\rho_i(x_1),\ldots,\rho_i(x_h)$ be the configurations 
associated by these partial runs with the nodes $x_1,\ldots,x_h$. 
Moreover, suppose that for all $j=1,\ldots,h$, we have
$$
  \rho_i(x_j) ~=~ \big\{\, \bar{\cA}\ang{t,U}[i](x_j) ~:~ U\subseteq\dom(t) \,\big\} \ .
$$ 
The definition of the transition relation of $\cA'_i$ (cf. item (1) above) 
defines a unique possible transition of the form $(S,C,\rho_i(x_1),\ldots,\rho_i(x_h))$ 
that can be executed at node $x$ with label $C=(d,a,\rho_{i-1}(x))$. More precisely, 
the set $S$ contains all and only the configurations of the form $(b,q)$ for which there 
exist $(b,q')\in \rho_{i-1}(x)$, $(b_1,q_1)\in S_i(x_1)$, $\ldots$, and $(b_h,q_h)\in S_i(x_h)$ 
such that $(q,(d,a,b,q'),q_1,\ldots,q_h)\in T_i$. Note, in particular, that thanks 
to the projectability of $\cA_i$, this set $S$ contains only pairwise orbit-distinct 
elements, and hence belongs to the configuration space $Q'_i$ of $\cA'_i$.
We can thus prolong the partial run on $\ang{t,\rho_{i-1}}$ by letting $\rho_i(x) = S$.
A close inspection to the definition of $S$ and the inductive hypothesis finally reveals 
that the equality ($\star$) holds in node $x$.

Similar constructions and arguments apply when $\cA_i$ is top-down deterministic -- 
the structural induction on $\ang{t,\bar{U}}$, in this case, starts from the root 
and goes downward.
\end{proof}

The above claim and the definitions of the sets of final configurations of the FMA
$\cA'_1,\ldots,\cA'_\ell$ immediately imply that the cascade product 
$\bar{\cA}'=\cA'_1*\ldots*\cA'_\ell$ recognizes the projection $L'$ of the language
$L$ recognized by $\bar{\cA}=\cA_1*\ldots*\cA_\ell$.

We now turn towards proving that the cascade product $\bar{\cA}'=\cA'_1*\ldots*\cA'_\ell$
is projectable. Recall that every FMA $\cA'_i$ is bottom-up deterministic or top-down 
deterministic and hence the first condition of Definition \ref{def:projectable-fma}
is satisfied. Moreover, for $i=\ell$, Claim \ref{claim:fma-subset-construction}
implies that for every data tree $t$, there exist (necessarily unique) runs 
$\rho_1,\rho_2,\ldots,\rho_\ell$ of $\cA_1,\cA_2,\ldots,\cA_\ell$ on the data 
trees $t$, $\ang{t,\rho_1}$, $\ldots$, $\ang{t,\rho_{\ell-1}}$. In particular,
the product of these runs can be seen a run $\bar{\cA}'\ang{t}$ of the FMA $\bar{\cA}'$.
This proves the second condition of Definition \ref{def:projectable-fma}.
It remains to verify the last condition. For this, it is interesting to give 
a proof for the most general case, namely, to assume that $A=A'\times B^m$ and 
that $\bar{\cA}$ is projectable over $B^{m+1}$, and to prove that $\bar{\cA}'$ 
is projectable over $B^m$. 
We thus consider data trees of the form $\ang{t',\bar{U}}$, where $\bar{U}=(U_1,\ldots,U_m)$ 
is an $m$-tuple of predicates. As usual, we denote by $\bar{\cA}'\ang{t,\bar{U}}$ the 
unique run of $\bar{\cA}'$ on $\ang{t',\bar{U}}$. Claim \ref{claim:fma-subset-construction} 
implies that for all nodes $x$, 
$$
  \bar{\cA}'\ang{t',\bar{U}}(x) 
  ~=~ \prod_{j=1}^n \rho_j(x) 
  ~=~ \prod_{j=1}^n \big\{\, \bar{\cA}\ang{t,\bar{U},U_{m+1}}[j](x) ~:~ U_{m+1}\subseteq\dom(t) \,\big\} 
  \ . 
$$
In particular, if we have two configurations $\bar{\cA}'\ang{t',\bar{U}}(x)$ and
$\bar{\cA}'\ang{t',\bar{V}}(x)$ in the same orbit, for some tuples of predicates
$\bar{U},\bar{V}$ and some node $x$, then we know that there exists a renaming
$\tau$ such that, for all $j=1,\ldots,\ell$, 
$$
  \big\{\, \bar{\cA}\ang{t,\bar{U},U_{m+1}}[j](x) ~:~ U_{m+1}\subseteq\dom(t) \,\big\}
  ~~=~~ 
  \big\{\, \tau\big(\bar{\cA}\ang{t,\bar{V},V_{m+1}}[j](x)\big) ~:~ V_{m+1}\subseteq\dom(t) \,\big\} \ .
$$
Moreover, since each of the two sets above contain pairwise orbit-distinct elements
and since $\bar{\cA}$ is projectable over $B^{m+1}$, we must conclude that the two 
sets are equal. In particular, this proves that 
$\bar{\cA}'\ang{t',\bar{U}}(x) \:=\: \bar{\cA}'\ang{t',\bar{V}}(x)$
and hence $\bar{\cA}'$ is projectable over $B^m$.
\end{proof}

To complete the proof of Theorem \ref{th:semi-rigid-inside-fma}, there is still one property 
that we need to verify, which concerns the translation of data tests guarded by semi-rigid 
formulas, namely, formulas of the form $\alpha(x,y) \:\et\: \beta(x,z) \:\et\: y\sim z$. 
The outline of the translation is roughly as follows. First, we inductively translate the 
guards $\alpha(x,y)$ and $\beta(x,z)$ into two projectable cascade products $\bar\cA$ and 
$\bar\cB$ over the alphabet $D\times A\times B^2$, where the predicate corresponding to the 
first (resp., second) copy of $B$ encodes the interpretation for the variable $x$ (resp., 
$y$ or $z$, depending on the formula). We then translate the data test $y\sim z$ into an 
equivalent (not projectable) FMA $\cC$ over the alphabet $D\times A\times B^2$. Finally, 
we aim at proving that the language defined by $\alpha(x,y) \:\et\: \beta(x,z) \:\et\: y\sim z$
is recognized by a suitable intersection of the cascade products $\bar\cA$, $\bar\cB$, $\bar\cC$.
Before doing this, however, we need to further process the cascade products $\bar\cA$ and 
$\bar\cB$ in order to enforce a stronger notion of projectability, called sink-reduced 
projectability, which will be then shown to be compatible with intersection of a
non-projectable FMA. As usual, we also need to apply cylindrification in order to 
get languages over the same alphabet $D\times A\times B^3$ that correctly refer to 
the variables $x,y,z$ of the formulas $\alpha(x,y)$, $\beta(x,z)$, $y\sim z$.

Below, we recall the notion of sink configuration, which is essentially a (final or non-final) 
configuration that cannot be left, and we generalize this notion to cascade products of FMA. 
We then give the definition of sink-reduced projectability.

\begin{definition}\label{def:sink-configuration}
Let $\cA=(\Sigma,Q,F,T)$ be a bottom-up deterministic (resp., top-down deterministic) FMA.
We say that a configuration $q\in Q$ is a \emph{sink} in $\cA$ if $q$ has empty memory and 
for all transitions $(q_0,c,q_1,\ldots,q_h)\in T$, if $q_i=q$ for some $1\le i\le h$, then 
$q_0=q$ (resp., if $q_0=q$, then $q_i=q$ for all $1\le i\le h$).
\par\noindent
Similarly, by identifying the configurations of a cascade product $\bar\cA=\cA_1*\ldots*\cA_\ell$ 
with $\ell$-tuples of configuations of the FMA $\cA_1,\ldots,\cA_\ell$, we say that 
$\bar{q}=(q_1,\ldots,q_h)$ is a \emph{sink} in $\bar\cA$ if each $q_i$ is a sink in $\cA_i$.
\end{definition}

\begin{definition}\label{def:sink-reduced-projectability}
A cascade product $\bar\cA$ over the alphabet $D\times A\times B^2$ is 
\emph{sink-reduced projectable} if it is projectable and, in addition, for all data 
trees $t$ over $D\times A$, all predicates $U,U'\subseteq\dom(t)$, and all nodes $y,y',z$, 
if the two configurations $\bar\cA\ang{t,U,\{y\}}(z)$ and $\bar\cA\ang{t,U',\{y'\}}(z)$ 
coincide, then $y=y'$ or both configurations are sink in $\bar\cA$.
\end{definition}

We now prove the following:

\begin{lemma}\label{lemma:sink-reduced-projectability}
Let $\varphi(x,y)$ be a formula of semi-rigidly guarded \MSO and let $\bar\cA$ be a projectable
cascade product that recognizes the language $\intr{\varphi}$ over the alphabet $D\times A\times B^2$. 
If $x$ determines $y$ in $\varphi(x,y)$, then one can compute from $\bar\cA$ a sink-reduced 
projectable cascade product $\bar\cA'$ equivalent to $\bar\cA$.
\end{lemma}

\begin{proof}
Let $\bar\cA=\cA_1*\ldots*\cA_\ell$. The proof goes by induction on $\ell$ and consists of
transforming each partial cascade product $\cA_1*\ldots*\cA_i$ into one that is sink-reduced.
Each transformation is achieved by grouping together those control states of $\cA_i$ that 
cannot be distinguished in terms of acceptance of some continuation of the input, expanded
with the induced computations of the underlying FMA $\cA_1,\ldots,\cA_{i-1}$ -- intuitively,
the transformation can be seen as a variant of minimization of finite automata based on
the one-sided Myhill-Nerode equivalence.
\gabriele{To edit from here}
Formally, we define the equivalence $\sim_i$ over the control states of $\cA_i$ in such 
a way that $q\sim q'$ iff, for all data trees $t$ over $D\times A\times B^2$,

We call these states \emph{trap states}.
Computing trap states can be done again by a simple reachability analysis. Formally, one defines $\cA'$
as the FMA obtained from $\cA$ by introducing a new control state $q_{\mt{sink}}$, with memory size $0$,
by redirecting to $q_{\mt{sink}}$ all the transitions that reach some trap state (erasing at same time 
the entire memory), and finally pruning the trap states. Clearly, the thus defined automaton $\cA'$ is 
equivalent to $\cA$. Moreover, it is easy to see that is deterministic, complete, and projectable.

We need to prove that $\cA'$ is $0$-reduced projectable. For this we use the fact that the automaton
recognizes the language $\intr{\varphi}$, which is defined by the {\sl backward-rigid} formula $\varphi(x,y)$. 
Let $w\in (D\times A)^*$ be a data word and let $x,x'\in\dom(w)$ be two positions in it. By way of contradiction, 
we assume that (i) $x\neq x'$ and (ii) the two configurations $\cA'(\ang{w,\{x\},\emptyset})$ and 
$\cA'(\ang{w,\{x'\},\emptyset})$ concide but they are not the $0$-configuration $(q_{\mt{sink}},\emptystr)$. 
From this we argue that $\varphi(x,y)$ is not backward-rigid. 
Since the configuration $\cA'(\ang{w,\{x\},\emptyset})$ is not a $0$-configuration, it can reach a final 
configuration, namely, there is an expanded data word $\ang{v,U_1,U_2}\in(D\times A\times B^2)$ such that
$$
  \ang{w,\{x\},\emptyset}\cdot\ang{v,U_1,U_2} \in \sL(\cA').
$$
Similarly, since $\cA'(\ang{w,\{x\},\emptyset})=\cA'(\ang{w,\{x'\},\emptyset})$, we have that
$$
  \ang{w,\{x'\},\emptyset}\cdot\ang{v,U_1,U_2} \in \sL(\cA').
$$
Since $x\neq x'$, this is against the backward-rigidity of the formula $\varphi(x,y)$ defining $\sL(\cA')$.
This completes the proof of Claim 3.
\end{proof}

We now argue that the data language $\intr{\varphi(x,y)\et x\sim y}$ is recognized by a projectable FMA. 
We denote by $\cA'$ a $0$-reduced projectable FMA recognizing $\intr{\varphi}$. Moreover, we denote by
$\cB$ the ``minimal'' deterministic FMA that recognizes $\intr{x\sim y}$. The automaton $\cB$ has four
control states: 
\begin{enumerate}
  \item a control state $q_{\mt{wait}}$, with empty memory, for parsing the prefix up to $\min(x,y)$,
  \item a control state $q_{\mt{check}}$, with memory size $1$, for parsin the infix from $\min(x,y)+1$ to $\max(x,y)$,
  \item a final control state $q_{\mt{accept}}$, with empty memory, for parsing the suffix from $\max(x,y)+1$ to the end,
        in the case where the data test $x\sim y$ was successful,
  \item a sink control state $q_{\mt{reject}}$, with empty memory, for parsing the same suffix above, but in the 
        case where the data test $x\sim y$ failed.
\end{enumerate}
One can construct an FMA $\cC$ recognizing $\intr{\varphi(x,y)\et x\sim y}$ using a suitable product between 
the $0$-reduced projectable FMA $\cA'$ and the deterministic (but not projectable) FMA $\cB$ described above. 
This product is very similar to the $0$-collapse product of orbit finite data monoids (see the proof of Lemma 
\ref{lemma:reduced-to-projectable} in Section \ref{app:logic2monoids}). Intuitively, $\cC$ mimics the computations
of $\cA'$ and $\cB$ on the input word, but as soon as $\cA'$ reaches the (unique) $0$-configuration, the component
that simulates the computation of $\cB$ is reset to a special void configuration with empty memory. Of course 
the defined FMA $\cC$ is deterministic and complete, as $\cA'$ and $\cB$ are so. 

We verify that $\cC$ is projectable. Consider a data word $w\in (D\times A)^*$ and some predicates 
$U_1,U_2,V_1,V_2\subseteq\dom(u)$. Suppose that the configurations $\cC(\ang{u,U_1,U_2})$ and $\cC(\ang{u,V_1,V_2})$ 
contain the same control state. We consider also the configurations reached by $\cA'$ after parsing $\ang{u,U_1,U_2}$ 
and $\ang{u,V_1,V_2}$. In particular, we distinguish between the case where $\cA'(\ang{u,U_1,U_2})$ is the 
$0$-configuration (and hence $\cA'(\ang{u,V_1,V_2})$ as well) and the case where $\cA'(\ang{u,U_1,U_2})$ is 
not the $0$-configuration (and hence $\cA'(\ang{u,V_1,V_2})$ as well). In the former case, we immediate obtain 
that the two configurations reached by $\cC$ after parsing $\ang{u,U_1,U_2}$ and $\ang{u,V_1,V_2}$ must coincide 
(this is because the components of these two configurations that simulate $\cB$ have been reset as $\cA'$ has 
reached the $0$-configuration). 
In the latter case, since $\cC(\ang{u,U_1,U_2})$ and $\cC(\ang{u,V_1,V_2})$ contain the same control state, 
we have the same for the configurations $\cA'(\ang{u,U_1,U_2})$ and $\cA'(\ang{u,V_1,V_2})$. Moreover, since 
$\cA'$ is projectable, we get $\cA'(\ang{u,U_1,U_2})=\cA'(\ang{u,V_1,V_2})$. So the only way the configurations 
$\cC(\ang{u,U_1,U_2})$ and $\cC(\ang{u,V_1,V_2})$ can differ is in the components that simulate $\cB$. Below, 
we analyse these components and we argue that they coincide:
\begin{enumerate}
  \item If $U_1=U_2=\emptyset$, then $\cB(\ang{u,U_1,U_2})=(q_{\mt{wait}},\emptystr)$. Moreover, since
        $\cC(\ang{u,U_1,U_2})$ and $\cC(\ang{u,V_1,V_2})$ share the same control state, the two components
        of $\cC(\ang{u,U_1,U_2})$ and $\cC(\ang{u,V_1,V_2})$ for simulating $\cB$ encode the same control state of $\cB$.
        In particular, it follows that $\cB(\ang{v,V_1,V_2})$ has control state $q_{\mt{wait}}$ and hence 
        $\cB(\ang{u,U_1,U_2})=\cB(\ang{v,V_1,V_2})$.
  \item If both $U_1$ and $U_2$ are non-empty, then $\cB(\ang{u,U_1,U_2})$ is either $(q_{\mt{accept}},\emptystr)$ 
        or $(q_{\mt{reject}},\emptystr)$.
        Using arguments similar to the previous case, one obtains $\cB(\ang{u,U_1,U_2})=\cB(\ang{v,V_1,V_2})$.
  \item If $U_1\neq\emptyset$ and $U_2=\emptyset$, then clearly $U_1$ is a singleton of the form $\{x\}$
        and the configuration $\cB(\ang{u,U_1,U_2})$ contains the control state $q_{\mt{check}}$ and the data value at
        the position $x$ of $u$. Similarly, since the configurations $\cB(\ang{u,U_1,U_2})$ and $\cB(\ang{u,V_1,V_2})$
        share the same control state, we have that $V_1$ is a singleton of the form $\{x'\}$ and $V_2=\emptyset$.
        Moreover, since the two configurations $\cA'(\ang{u,U_1,U_2})$ and $\cA'(\ang{u,U_1,U_2})$ coincide
        and they are different from the $0$-configuration, we have $x=x'$. This implies
        $\cB(\ang{u,U_1,U_2})=\cB(\ang{v,V_1,V_2})$.
  \item The last case $U_1=\emptyset$ and $U_2\neq\emptyset$ is similar to the previous one.
\end{enumerate}
It follows that $\cC(\ang{u,U_1,U_2})=\cC(\ang{u,V_1,V_2})$. This shows that $\cC$ is a projectable FMA.


\begin{proof}[Proof of Theorem \ref{th:semi-rigid-inside-fma}]
As previously mentioned, the proof that any backward-rigidly guarded MSO formula $\varphi$ 
can be translated into an equivalent deterministic (and projectable) FMA goes by structural
induction on $\varphi$, using the closures of deterministic projectable FMA under projection,
complement, intersection. For the backward-rigidly guarded data tests one uses the construction
just mentioned above.
\end{proof}


...BLA BLA BLA...

\begin{proposition}
There is a language recognized by a deterministic FMA that cannot be 
defined in backward-rigidly guarded \MSO.
\end{proposition}

\begin{proof}
Consider the language $L''$ of data words of the form
$$
  d_1~d_2~\ldots~d_n
$$
for which there is a sequence of indices $1=i_1<i_2<\ldots<i_k=n$ satisfying 
$d_{i_j+1}=d_{i_{j+1}}$ for all $1\le j<k$ and $d_{i_j+1}\neq d_h$ for all
$i_j+1<h<i_{j+1}$ \footnote{This language is a variant of an example given 
in \cite{graph_reachability_with_pebbles} to study data languages recognized 
by pebble automata.}.

It is easy to see that $L''$ is recognized by a deterministic FMA that uses 
only one register: at each phase, the automaton stores the value under the 
current position and then moves to the right searching for the another occurrence 
of the stored value -- if it does not find such an occurrence, then it rejects, 
otherwise, as soon as the occurrence is found, the automaton moves to the next 
position to the right (if any, otherwise it accepts) and starts a new phase. 

Below, we fix a generic formula $\varphi$ of backward-rigidly guarded MSO and 
we show that it cannot define the language $L''$. For this, we let $k$ be the 
number of occurrences of data comparisons of the form $\alpha(y,z)\et y\sim z$ 
in $\varphi$. We then consider a family of data words of the form
$$
  w_n ~=~ 0~u_n^{(0)}~0~~1~u_n^{(1)}~1~~\ldots~~n~u_n^{(n)}~n
$$
where $n$ ranges over the positive natural numbers, each word $u_n^{(i)}$ has 
length exactly $n$, and the juxtaposition $u_n^{(0)}\cdot u_n^{(1)}\cdot\ldots\cdot u_n^{(n)}$ 
contains pairwise distinct values from the set $\bbN\setminus\{0,\ldots,n\}$ 
(therefore, the only equalities that hold in $w_n$ are those between the 
occurrences of the data values $0,\ldots,n$). Without loss of generality, 
we also assume that for every backward-rigidly guarded data test
$\alpha(x,y) \et x \sim y$ in $\varphi$, the guard $\alpha(x,y)$ holds 
{\sl only if} $x$ is interpreted by a position to the left of the position 
that interprets $y$.

Using an encoding similar to the proof of Corollary \ref{cor:rigidification}, 
one can turn each data word $w_n$ into a classical word $w_n^*$ over the 
finite alphabet $\{0,1\}^k$ where every position $y$ of $w_n^*$ is labeled 
by a $k$-tuple of boolean values, each of them representing the ``observable'' 
equality between the value at the position $y$ of $w_n$ and the value at the 
unique position $x$ determined from $y$ via the backward-rigid guard of a 
corresponding data test $\alpha(x,y)\et x\sim y$ of $\varphi$. 
Accordingly, we can rewrite every sub-formula $\beta$ of $\varphi$ into a 
formula $\beta^*$ of standard MSO by replacing each backward-rigid guard 
$\alpha(x,y)$ of a data test in $\beta$ by a fresh unary predicate
$$
  [\alpha^{\sim}](y).
$$
Clearly, we have that for every $n$, every backward-rigid guard $\alpha(x,y)$ 
of $\varphi$, and every position $x<\len{w_n}$ in $w_n$,
$$
  w_n\sat\alpha(x,\len{w_n}) \qquad\text{iff}\qquad w_n^*\sat\alpha^*(x,\len{w_n}).
$$
Moreover, one can prove that there is a number $n_\alpha$, which only depends 
on $\alpha$, such that for all $n\in\bbN$ and all pairs of positions $1\le x<y\le\len{w_n}$,
\begin{align*}
  w_n^*\sat\alpha^*(x,y) \qquad\text{implies}\qquad 1\le x\le n_\alpha \vel y-n_\alpha\le x<y. \tag{$\star$}
\end{align*}
The proof of $\star$ is by structural induction on the number of nested rigid guards. 
The statement holds because the word $w_n$ is over the alphabet $D$, that is, there 
are no labels from a finite alphabet that can be used to ``rigidly jump'' far from 
the original position $y$ and from the endpoints of the word. We omit the details.

If we let $y=\len{w_n}=(n+1)^2$ in the above implication and we consider 
a sufficiently large $n$ (i.e. $n>n_\alpha$ for all backward-rigid guards $\alpha$ of $\varphi$), 
we obtain that there is no backward-rigid guard $\alpha(x,y)$ in $\varphi$ that, given the 
last position $y$ in $w_n$, which carries the value $n$, determines the position 
$x$ of the other occurrence of the value $n$ in $w_n$. This shows that 
$$
  w_n\sat\varphi \qquad\text{iff}\qquad w_n^*\sat\varphi^* \qquad\text{iff}\qquad w_n[\len{w_n}\mapsto n+1]\sat\varphi
$$
where $w_n[\len{w_n}\mapsto n+1]$ is the data word obtained from $w_n$ by 
relabeling the last position with the fresh value $n+1$. Since $w_n\in L''$
and $w_n[\len{w_n}\mapsto n+1]\nin L''$, this shows that $\varphi$ does not
define the language $L''$.
\end{proof}





\subsection{$\exists$Backward-rigidly guarded MSO} 

We do not have a candidate logic that corresponds precisely to deterministic FMA. 
However, we are able to characterize the larger class of languages recognized by 
non-deterministic FMA. The logic for this class is obtained from backward-rigidly 
guarded MSO by allowing the guards to use additional second-order variables (which 
however needs to be quantified existentially in the outermost part of the formula). 
The logic, abbreviated \emph{$\exists$backward-rigidly guarded MSO}, consists of  
the formulas $\exists \bar{Z}.~ \varphi$, with $\varphi$ is generated by the grammar
\begin{align*}
  \varphi := \exists x.~ \varphi \,\mid\, \exists Y.~ \varphi \,\mid\, x\!<\!y \,\mid\, 
             a(x) \,\mid\, x\!\in\! Y \,\mid\, \neg\varphi \,\mid\, \varphi \!\et\! \varphi \,\mid\,
             \varphi_{\exists\text{backward}}(x,y,\bar{Z}) \!\et\! x \!\sim\! y
\end{align*}
\gabriele{Shall we explain what is $\max(x,y)$??! (see reviewer comment)}
where $\varphi_{\exists\text{backward}}$ is a formula from the same grammar that 
determines $\min(x,y)$ from $\max(x,y)$ and $\bar{Z}$, and where the quantifications 
are over variables different from $\bar{Z}$ (the variables $\bar{Z}$ are quantified 
only in the outermost part of $\exists \bar{Z}.~ \varphi$).

\begin{theorem}\label{thm:existbackward-rigid-mso}
A language is definable in $\exists$backward-rigidly guarded MSO iff it is recognizable 
by non-deterministic FMA.
\end{theorem}   


\begin{proof}
Having established Lemma \ref{lemma:backward-rigid-to-automata}, the translation from 
an $\exists$backward-rigidly formula $\exists \bar{Z}.~ \varphi$ to an equivalent non-deterministic 
FMA that recognizes the language $L=\intr{\exists \bar{Z}.~ \varphi}$ is straightforward. For this,
we first translate $\varphi$ into a {\sl deterministic} FMA $\cA$ that recognizes the language 
$L'=\intr{\varphi}$ (note that this language is over the alphabet $D\times A\times B^m$, where 
$m=\len{\bar{Z}}$). After that, we project $\cA$ onto the alphabet $D\times A$: the resulting
automaton is a non-deterministic FMA that guesses the correct interpretation for the second-order 
variables $\bar{Z}$ on any input data word that belongs to the language $L=\intr{\exists \bar{Z}.~ \varphi}$.


\medskip
We now prove the converse direction, that is, we translate a non-deterministic FMA 
$\cA=(D,A,k,Q_0,\ldots,Q_k,T,I,F)$ into an equivalent $\exists$backward-rigidly guarded MSO 
sentence. As in the classical theory, the proof is based on an encoding a successful run of 
$\cA$ on the input word. For this we need a second-order variable $Z_t$ for each transition 
rule $t\in T$ of $\cA$. The formula that defines the recognized language $\sL(\cA)$ begins 
with a block of existential monadic quantifiers of the form $\exists \bar{Z}$, where 
$\bar{Z}=(Z_t)_{t\in T}$. The matrix of the desired formula (i.e. the part after 
the block of existential monadic quantifiers) is a backward-rigidly guarded MSO 
formula $\varphi(\bar{Z})$ that checks that the interpretations of the variables
$\bar{Z})$ encode a valid run of $\cA$. 

Formally, given an input data word $w=(d_1,a_1)\ldots(d_n,a_n)$, the formula $\varphi(\bar{Z})$ checks that:
\begin{enumerate}
  \item For all positions $1\le x\le\len{w}$, exactly one variable $Z_t$ with $t\in T$ holds at $x$
        (i.e., $\forall x.~ \bigvee_{t\in T}x\in Z_t\et\bigvee_{t\neq t'\in T} x\nin Z_t\vel x\nin Z_{t'}$).
        We will say that a transition rule $t$ is \emph{encoded} at a position $x$ if $x\in Z_t$ holds.
  \item For all positions $1\le x<\len{w}$, the target state of the transition rule encoded at position $x$ 
        coincides with the source state of the transition rule encoded at position $x+1$ 
        (i.e., $\forall x.~ \bigvee_{t=(p,\theta,E,q),t'=(q,a,\theta',E',q')\in T} x\in Z_t\et x+1\in Z_{t'}$).
  \item The transition rule encoded at the first position of the word starts with an intial control state and 
        the transition rule encoded at the last position of the word ends with a final control state.
  \item For all positions $1\le x\le\len{w}$, if $t=(p,a,\theta,E,q)$ is the transition rule encoded at position $x$,
        then $a=a_x$, where $a_x$ is the symbol that appears at position $x$ of the input word.
  \item For all positions $1\le x\le\len{w}$, if $t=(p,a,\theta,E,q)$ is the transition rule encoded at position $x$,
        then $\theta$ is the isomorphism type of $r_{x-1}\cdot d_x$, where $r_x$ is the memory content at
        position $x-1$ in the encoded run of $\cA$ and $d_x$ is the data value at position $x$ of the input word .

        To see how this check is done, consider an example of a partial run of $\cA$:
        $$
          (q_0,r_0) ~\trans{(d_1,a_1)}~ (q_1,r_1) ~\trans{(d_2,a_2)}~ \ldots ~\trans{(d_{x-1},a_{x-1})}~ (q_{x-1},r_{x-1}).
        $$
        For each register $i$ of $r_{x-1}$, we need to determine the ``provenance'' of the value 
        $r_{x-1}[i]$ in the prefix $(d_1,a_1)(d_2,a_2)\ldots(d_{x-1},a_{x-1})$ of the input word,
        namely, we need to locate some position $y\le x-1$ such that $d_y=r_{x-1}[i]$.
        We thus reconstruct, for each $z\le x-1$, the position $f_{x,i}(z)$ of the occurrence of 
        $r_{x-1}[i]$ (if any) in the memory $r_z$. This can be done by a suitable formula that 
        first guesses some monadic variables $W_1,\ldots,W_k$ encoding the partial function 
        $f_{x,i}(z)$, and then verifies, using the run encoded by the variables $\bar{Z}$, 
        that the guess is correct. One can also do this using only first-order quantifications,
        since the partial function $f_{x,i}(z)$ can only decrease as $z$ increases; however,
        we prefer not to discuss this option in detail.
        We then compute the leftmost position $y$ such that $f_{x,i}(z)$ is defined on all $z=y,\ldots,x-1$.
        Clearly, this implies $d_y=r_{x-1}[i]$. 

        The formula that determines $y$ from $x$ using $\bar{Z}$ is of the form
        $$
          \alpha_i(y,x,\bar{Z}) ~\eqdef~ \beta_i(y,x,\bar{Z}) \et \forall y'.~ y'<y\then\neg\beta_i(y',x,\bar{Z})
        $$ 
        where 
        \begin{align*}
          \beta_i(y,z,\bar{Z}) & ~\eqdef~ \exists W_1,\ldots,W_k.~ \forall z.~ \\
                               & \quad y\le z\le x-1 \then    
                                 \Big(\bigvee_{1\le j\le k}z\in W_j \et \neg\bigwedge_{1\le j<j'\le k}z\in W_j\et z\in W_{j'} \\
                               & \quad \phantom{y\le z\le x-1} \et 
                                 \!\!\!\!\!\!\bigvee_{\begin{smallmatrix}1\le j\le k,~ p\in Q_j \\ t=(p,a,\theta,E,q)\in T \end{smallmatrix}}\!\!\!\!\!\!\!\!\!\!\!\!
                                 z\in Z_t \et z\in W_j \et z-1\in W_{j-\len{E\cap\{1,\ldots,j\}}}\Big)
        \end{align*}
        Note that $\alpha_i(y,x,\bar{Z})$ is an $\exists$backward-rigid formula.
        We can thus use $\alpha_i$ as a guard to test equality between the 
        data value $d_x$ at position $x$ and the data value $d_i$ ($=r_{x-1}[i]$) at position $y$.
        
        Using the above constructions we can check that the isorphism type 
        of the transition rule encoded at position $x$ coincides with the isomorphism type of $r_{x-1}\cdot d_x$.
\end{enumerate}
Thus $\varphi(\bar{Z})$ is a formula that verifies that the sequence of transition rules
encoded by $\bar{Z}$ is a valid run of $\cA$ on the input word. Hence
$\exists \bar{Z}.~ \varphi(\bar{Z})$ is a $\exists$backward-rigidly guarded MSO sentence 
that defines the language $\sL(\cA)$ recognized by $\cA$.
\end{proof}





As it happens for rigidly guarded MSO logic, one can derive from Theorem \ref{thm:existbackward-rigid-mso} 
the following decidability results:

\begin{corollary}\label{cor:existbackward-rigid-mso}
The satisfiability problem for $\exists$backward-rigidly guarded MSO is decidable. 
Moreover, one can decide whether a formula belongs to the $\exists$backward-rigidly guarded MSO,
and in this case whether the formula is $\exists$backward-rigid.
\end{corollary}

\begin{proof}
By Theorem \ref{thm:existbackward-rigid-mso}, any formula of $\exists$backward-rigidly guarded MSO 
can be effectively transformed into a non-deterministic FMA. Satisfiability of $\exists$backward-rigidly 
guarded MSO then corresponds to non-emptiness of languages recognized by non-deterministic FMA. The
latter problem is known to be decidable from \cite{finite_memory_automata}.

The second claim follows from arguments similar to the proof of Corollary \ref{cor:decidability-logic},
that is, one can inductively check that every sub-formula satisfies the syntactical restrictions 
given by the grammar of $\exists$backward-rigidly guarded MSO. For the sub-formulas $\alpha(x,y,\bar{Z})$ 
that are guards of data equality tests, one has also to verify that $\alpha$ is $\exists$backward-rigid
by checking the validity of the formula
$$
  \alpha^{\exists\text{backward?}} ~\eqdef~ \forall x,x',y,\bar{Z}.~ \alpha(x,y,\bar{Z}) \et \alpha(x',y,\bar{Z}) \then x=x'.
$$\qedhere
\end{proof}


\subsection{Extension to trees} 

It is also easy to generalize both Theorem \ref{thm:existbackward-rigid-mso} and Corollary
\ref{cor:existbackward-rigid-mso} to data {\sl tree} languages recognized by non-deterministic 
finite memory tree automata \cite{finite_memory_tree_automata}. For this we use a natural variant 
of $\exists$backward-rigidly guarded MSO on data trees. The guarded tests in this case are 
of the form 
$$
  \varphi_{\exists\mt{downward}}(x,y,\bar{Z})\et \varphi'_{\exists\mt{downward}}(x,z,\bar{Z})\et y\sim z
$$
where $\varphi_{\exists\mt{downward}}(x,y,\bar{Z})$ 
(resp. $\varphi'_{\exists\mt{downward}}(x,z,\bar{Z})$) 
is a formula in the logic that determines the position $y$ (resp., $z$) from an ancestor $x$ in the
data tree and the second-order variables $\bar{Z}$. This logic happens to be equivalent
with the natural extension of non-deterministic FMA to trees.

%\margincomment{Perhaps this last paragraph should go to the conclusions}
Finally, it is natural to look for effective characterizations of data languages that are both 
recognizable by non-deterministic FMA and definable in (unrestricted) FO. However, it is known 
that such characterization cannot be achieved: in \cite{automata_vs_logics} it has been shown 
that the problem of determining whether a language recognized by a non-deterministic FMA is 
definable in FO is undecidable. The problem of characterizing FO within the class of languages 
recognizable by deterministic FMA is still open.

